A Class of Multirate Infinitesimal GARK Methods

Differential equations arising in many practical applications are characterized by multiple time scales. Multirate time integration seeks to solve them efficiently by discretizing each scale with a different, appropriate time step, while ensuring the overall accuracy and stability of the numerical solution. In a seminal paper Knoth and Wolke (APNUM, 1998) proposed a hybrid solution approach: discretize the slow component with an explicit Runge-Kutta method, and advance the fast component via a modified fast differential equation. The idea led to the development of multirate infinitesimal step (MIS) methods by Wensch et al. (BIT, 2009.)G\"{u}nther and Sandu (BIT, 2016) explained MIS schemes as a particular case of multirate General-structure Additive Runge-Kutta (MR-GARK) methods. The hybrid approach offers extreme flexibility in the choice of the numerical solution process for the fast component. This work constructs a family of multirate infinitesimal GARK schemes (MRI-GARK) that extends the hybrid dynamics approachin multiple ways. Order conditions theory and stability analyses are developed, and practical explicit and implicit methods of up to order four are constructed. Numerical results confirm the theoretical findings. We expect the new MRI-GARK family to be most useful for systems of equations with widely disparate time scales, where the fast process is dispersive, and where the influence of the fast component on the slow dynamics is weak.

==> coupled_implicit_methods.tex <==
%%%%%%%%%%%%%%%%%%%%%%
\section{Ccoupled implicit methods}
%%%%%%%%%%%%%%%%%%%%%%

Recall \eqref{eqn:MIS-additive}. The idea is to solve implicitly for a predictive stage with abscissa $c_{i+1}$, then use it in the forcing of the fast stage. The first stage is explicit, and the second one is implicit. For example, for $c_{2i+1}=c_{2i}$ we have:
%
\begin{subequations}
%\label{eqn:MIS-impl-additive}
%
\[
\begin{array}{c|c|c|c|c|c}
  \Ys_{3i-2}  &\Ys_{3i-1}  & \Ys_{3i}   &  \Ys_{3i+1}   &  \Ys_{3i+2}   &  \Ys_{3i+3} \\
 \hline
c^{\{\s\}}_{i} & c^{\{\s\}}_{i+1} & c^{\{\s\}}_{i+1} & c^{\{\s\}}_{i+1} & c^{\{\s\}}_{i+2} & c^{\{\s\}}_{i+2}
\end{array}
\]

\begin{eqnarray}
%\label{eqn:MIS-impl-additive-first-stage}
&& \Ys_{1} = y_{n}, \\
%
&& \Ys_{2} = \Ys_{1} + H\,\sum_{j=1}^{2} \overline{\gamma}_{1,j} \, \funs\bigl( Y^{\{\s\}}_j \bigr), \\
%
%\label{eqn:MIS-impl-additive-explicit-stage}
\qquad\qquad&& 
\begin{cases}
v(0) = \Ys_{3i-2}, \\
 v' = \bigl(  c^{\{\s\}}_{3i} - c^{\{\s\}}_{3i-2} \bigr) \, \funf \left( v \right) + \sum_{j=1}^{3i-1} \gamma_{3i-1,j}\left(\frac{\theta}{H}\right) \, \funs\bigl( Y^{\{\s\}}_j \bigr) , \quad \theta \in  [0,  H],  \\
\Ys_{3i} = v(H), \qquad i=1,\dots,s^{\{\s\}}, 
\end{cases}
\\
%\label{eqn:MIS-impl-additive-implicit-stage}
&& \Ys_{3i+1} = \Ys_{3i} + H\,\sum_{j=1}^{3i+1} \overline{\gamma}_{3i,j} \, \funs\bigl( Y^{\{\s\}}_j \bigr), \\
&& \Ys_{3i+2} = \Ys_{3i+1} + H\,\sum_{j=1}^{3i+2} \overline{\gamma}_{3i+1,j} \, \funs\bigl( Y^{\{\s\}}_j \bigr), \\
%\label{eqn:MIS-impl-additive-solution}
&& y_{n+1} = \Ys_{s^{\{\s\}}+1}\,.
\end{eqnarray}
\end{subequations}

%%%%%%%%%%%%%%%%%%%%%%
\section{Fully coupled implicit methods}
%%%%%%%%%%%%%%%%%%%%%%

Consider the implicit scheme \eqref{eqn:MIS-impl-additive}, and modify the implicit slow stage \eqref{eqn:MIS-impl-additive-implicit-stage} such as to add the coupling with the fast system:
%
\begin{subequations}
\label{eqn:MIS-impl-additive-coupled}
%
\begin{eqnarray}
\label{eqn:MIS-impl-additive-first-stage-coupled}
&& \Ys_{1} = y_{n}, \\
%
\label{eqn:MIS-impl-additive-explicit-stage-coupled}
\qquad\qquad&& \begin{cases}
v(0) = \Ys_{2i-1}, \\
 v' = \bigl(  c^{\{\s\}}_{2i} - c^{\{\s\}}_{2i-1} \bigr) \, \funf \left( v \right) + \sum_{j=1}^{2i-1} \gamma_{2i-1,j}\left(\frac{\theta}{H}\right) \, \funs\bigl( Y^{\{\s\}}_j \bigr), \quad \theta \in  [0,  H],  \\
\Ys_{2i} = v(H), \qquad i=1,\dots,s^{\{\s\}}, 
\end{cases}
\\
\label{eqn:MIS-impl-additive-implicit-stage-coupled}
&& \Ys_{2i+1} = \Ys_{2i} + H\,\overline{\gamma}_{2i,i+1} \, \left( \funs\bigl( Y^{\{\s\}}_{2i+1} \bigr) +  \funf\bigl( Y^{\{\s\}}_{2i+1} \bigr)  \right)  \\
\nonumber
&& \qquad\qquad + H\,\sum_{j=1}^{2i} \overline{\gamma}_{2i,j} \, \funs\bigl( Y^{\{\s\}}_j \bigr) + H\,\sum_{j=1}^{2i} \beta_{2i,j} \, \funf\bigl( Y^{\{\s\}}_j \bigr), \\
\label{eqn:MIS-impl-additive-solution-coupled}
&& y_{n+1} = \Ys_{s^{\{\s\}}+1}\,.
\end{eqnarray}
\end{subequations}
%
At each stage the fast and the slow systems are solved together.


==> order_five_conditions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Coupling conditions of order 5}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{eqnarray*}
&& t^{\langle N,\cdot \rangle}_{5,2} ~~ b^T (A c) x c^2 = 1/10 \\
&1. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \Big( (\mathbf{A}^{\{f,s\}}\cdot \mathbf{c}^{\{s\}} ) \times \mathbf{c}^{\{f\}}\,^{\times 2}  \Big) = \frac{1}{10} \\
&2. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \Big( (\mathbf{A}^{\{s,f\}}\cdot \mathbf{c}^{\{f\}} ) \times \mathbf{c}^{\{s\}}\,^{\times 2}  \Big) = \frac{1}{10} \\
\end{eqnarray*}
\begin{eqnarray*}
&& t^{\langle N,\cdot \rangle}_{5,3} b^T (A c^2) x c = 1/15 \\
&3. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \Bigg( \Big( \mathbf{A}^{\{f,s\}}\cdot  \mathbf{c}^{\{s\}}\,^{\times 2} \Big) \times \mathbf{c}^{\{f\}}  \Bigg)  = \frac{1}{15}  \\
&4. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \Bigg( \Big( \mathbf{A}^{\{f,f\}}\cdot  \mathbf{c}^{\{f\}}\,^{\times 2} \Big) \times \mathbf{c}^{\{f\}}  \Bigg)  = \frac{1}{15}  \\
&5. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \Bigg( \Big( \mathbf{A}^{\{f,s\}}\cdot  \mathbf{c}^{\{s\}}\,^{\times 2} \Big) \times \mathbf{c}^{\{f\}}  \Bigg)  = \frac{1}{15}  \\
&6. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \Bigg( \Big( \mathbf{A}^{\{s,f\}}\cdot  \mathbf{c}^{\{f\}}\,^{\times 2} \Big) \times \mathbf{c}^{\{s\}}  \Bigg)  = \frac{1}{15}  \\
&7. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \Bigg( \Big( \mathbf{A}^{\{s,s\}}\cdot  \mathbf{c}^{\{s\}}\,^{\times 2} \Big) \times \mathbf{c}^{\{s\}}  \Bigg)  = \frac{1}{15}  \\
&8. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \Bigg( \Big( \mathbf{A}^{\{s,f\}}\cdot  \mathbf{c}^{\{f\}}\,^{\times 2} \Big) \times \mathbf{c}^{\{s\}}  \Bigg)  = \frac{1}{15}  \\
\end{eqnarray*}
\begin{eqnarray*}
&& t^{\langle N,\cdot \rangle}_{5,4} b^T ( (A^2 c) x c ) = 1/30 \\
&9. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \Big( \left( \mathbf{A}^{\{f,s\}} \cdot \mathbf{A}^{\{s,f\}}  \cdot \mathbf{c}^{\{f\}}  \right)  \times  \mathbf{c}^{\{f\}} \Big) = \frac{1}{30} \\
&10. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \Big( \left( \mathbf{A}^{\{f,f\}} \cdot \mathbf{A}^{\{f,s\}}  \cdot \mathbf{c}^{\{s\}}  \right)  \times  \mathbf{c}^{\{f\}} \Big) = \frac{1}{30} \\
&11. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \Big( \left( \mathbf{A}^{\{f,s\}} \cdot \mathbf{A}^{\{s,s\}}  \cdot \mathbf{c}^{\{s\}}  \right)  \times  \mathbf{c}^{\{f\}} \Big) = \frac{1}{30} \\
&12. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \Big( \left( \mathbf{A}^{\{s,f\}} \cdot \mathbf{A}^{\{f,f\}}  \cdot \mathbf{c}^{\{f\}}  \right)  \times  \mathbf{c}^{\{s\}} \Big) = \frac{1}{30} \\
&13. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \Big( \left( \mathbf{A}^{\{s,s\}} \cdot \mathbf{A}^{\{s,f\}}  \cdot \mathbf{c}^{\{f\}}  \right)  \times  \mathbf{c}^{\{s\}} \Big) = \frac{1}{30} \\
&14. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \Big( \left( \mathbf{A}^{\{s,f\}} \cdot \mathbf{A}^{\{f,s\}}  \cdot \mathbf{c}^{\{s\}}  \right)  \times  \mathbf{c}^{\{s\}} \Big) = \frac{1}{30} \\
\end{eqnarray*}
\begin{eqnarray*}
&& t^{\langle N,\cdot \rangle}_{5,4.5}~~ b^T (Ac) x (Ac) = 1/20 \\
&15. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \Big( \left( \mathbf{A}^{\{f,f\}} \cdot \mathbf{c}^{\{f\}}  \right)  \times  \Big( \left( \mathbf{A}^{\{f,s\}} \cdot \mathbf{c}^{\{s\}}  \right) \Big) = \frac{1}{20} \\
&16. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \Big( \left( \mathbf{A}^{\{f,s\}} \cdot \mathbf{c}^{\{s\}}  \right)  \times  \Big( \left( \mathbf{A}^{\{f,f\}} \cdot \mathbf{c}^{\{f\}}  \right) \Big) = \frac{1}{20} \\
&17. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \Big( \left( \mathbf{A}^{\{f,s\}} \cdot \mathbf{c}^{\{s\}}  \right)  \times  \Big( \left( \mathbf{A}^{\{f,s\}} \cdot \mathbf{c}^{\{s\}}  \right) \Big) = \frac{1}{20} \\
&18. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \Big( \left( \mathbf{A}^{\{s,f\}} \cdot \mathbf{c}^{\{f\}}  \right)  \times  \Big( \left( \mathbf{A}^{\{s,f\}} \cdot \mathbf{c}^{\{f\}}  \right) \Big) = \frac{1}{20} \\
&19. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \Big( \left( \mathbf{A}^{\{s,f\}} \cdot \mathbf{c}^{\{f\}}  \right)  \times  \Big( \left( \mathbf{A}^{\{s,s\}} \cdot \mathbf{c}^{\{s\}}  \right) \Big) = \frac{1}{20} \\
&20. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \Big( \left( \mathbf{A}^{\{s,s\}} \cdot \mathbf{c}^{\{s\}}  \right)  \times  \Big( \left( \mathbf{A}^{\{s,f\}} \cdot \mathbf{c}^{\{f\}}  \right) \Big) = \frac{1}{20} \\
\end{eqnarray*}
\begin{eqnarray*}
&& t^{\langle N,\cdot \rangle}_{5,5}~~ b^T A c^3 = 1/20 \\
&21. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \mathbf{A}^{\{f,s\}} \cdot  \mathbf{c}^{\{s\}} \,^{\times 3} = \frac{1}{20} \\
&22. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \mathbf{A}^{\{s,f\}} \cdot  \mathbf{c}^{\{f\}} \,^{\times 3} = \frac{1}{20} \\
\end{eqnarray*}
\begin{eqnarray*}
&& t^{\langle N,\cdot \rangle}_{5,6}~~ b^T A (Ac x c) = 1/40 \\
&23. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \mathbf{A}^{\{f,f\}} \cdot  \Big( (\mathbf{A}^{\{f,s\}}\cdot \mathbf{c}^{\{s\}} ) \times \mathbf{c}^{\{f\}} \Big) = \frac{1}{40} \\
&24. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \mathbf{A}^{\{f,s\}} \cdot  \Big( (\mathbf{A}^{\{s,f\}}\cdot \mathbf{c}^{\{f\}} ) \times \mathbf{c}^{\{s\}} \Big) = \frac{1}{40} \\
&25. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \mathbf{A}^{\{f,s\}} \cdot  \Big( (\mathbf{A}^{\{s,s\}}\cdot \mathbf{c}^{\{s\}} ) \times \mathbf{c}^{\{s\}} \Big) = \frac{1}{40} \\
&26. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \mathbf{A}^{\{s,f\}} \cdot  \Big( (\mathbf{A}^{\{f,f\}}\cdot \mathbf{c}^{\{f\}} ) \times \mathbf{c}^{\{f\}} \Big) = \frac{1}{40} \\
&27. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \mathbf{A}^{\{s,f\}} \cdot  \Big( (\mathbf{A}^{\{f,s\}}\cdot \mathbf{c}^{\{s\}} ) \times \mathbf{c}^{\{f\}} \Big) = \frac{1}{40} \\
&28. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \mathbf{A}^{\{s,s\}} \cdot  \Big( (\mathbf{A}^{\{s,f\}}\cdot \mathbf{c}^{\{f\}} ) \times \mathbf{c}^{\{s\}} \Big) = \frac{1}{40} \\
\end{eqnarray*}
\begin{eqnarray*}
&& t^{\langle N,\cdot \rangle}_{5,7}~~ b^T A^2 c^2 = 1/60 \\
&29. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \mathbf{A}^{\{f,f\}} \cdot  \mathbf{A}^{\{f,s\}} \cdot \mathbf{c}^{\{s\}}\,^{\times 2} = \frac{1}{60} \\
&30. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \mathbf{A}^{\{f,s\}} \cdot  \mathbf{A}^{\{s,f\}} \cdot \mathbf{c}^{\{f\}}\,^{\times 2} = \frac{1}{60} \\
&31. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \mathbf{A}^{\{f,s\}} \cdot  \mathbf{A}^{\{s,s\}} \cdot \mathbf{c}^{\{s\}}\,^{\times 2} = \frac{1}{60} \\
&32. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \mathbf{A}^{\{s,f\}} \cdot  \mathbf{A}^{\{f,f\}} \cdot \mathbf{c}^{\{f\}}\,^{\times 2} = \frac{1}{60} \\
&33. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \mathbf{A}^{\{s,f\}} \cdot  \mathbf{A}^{\{f,s\}} \cdot \mathbf{c}^{\{s\}}\,^{\times 2} = \frac{1}{60} \\
&34. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \mathbf{A}^{\{s,s\}} \cdot  \mathbf{A}^{\{s,f\}} \cdot \mathbf{c}^{\{f\}}\,^{\times 2} = \frac{1}{60} \\
\end{eqnarray*}
\begin{eqnarray*}
&& t^{\langle N,\cdot \rangle}_{5,8}~~ b^T A^3 c = 1/120 \\
&35. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \mathbf{A}^{\{f,f\}} \cdot  \mathbf{A}^{\{f, f\}} \cdot  \mathbf{A}^{\{f,s\}}  \cdot \mathbf{c}^{\{s\}} = \frac{1}{120} \\
&36. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \mathbf{A}^{\{f,f\}} \cdot  \mathbf{A}^{\{f, s\}} \cdot  \mathbf{A}^{\{s,s\}}  \cdot \mathbf{c}^{\{s\}} = \frac{1}{120} \\
&37. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \mathbf{A}^{\{f,s\}} \cdot  \mathbf{A}^{\{s, f\}} \cdot  \mathbf{A}^{\{f,f\}}  \cdot \mathbf{c}^{\{f\}} = \frac{1}{120} \\
&38. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \mathbf{A}^{\{f,s\}} \cdot  \mathbf{A}^{\{s, f\}} \cdot  \mathbf{A}^{\{f,s\}}  \cdot \mathbf{c}^{\{s\}} = \frac{1}{120} \\
&39. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \mathbf{A}^{\{f,s\}} \cdot  \mathbf{A}^{\{s, s\}} \cdot  \mathbf{A}^{\{s,f\}}  \cdot \mathbf{c}^{\{f\}} = \frac{1}{120} \\
&40. ~~&  \mathbf{b}^{\{f\}}\,^T \cdot \mathbf{A}^{\{f,s\}} \cdot  \mathbf{A}^{\{s, s\}} \cdot  \mathbf{A}^{\{s,s\}}  \cdot \mathbf{c}^{\{s\}} = \frac{1}{120} \\
&41. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \mathbf{A}^{\{s,f\}} \cdot  \mathbf{A}^{\{f, f\}} \cdot  \mathbf{A}^{\{f,f\}}  \cdot \mathbf{c}^{\{f\}} = \frac{1}{120} \\
&42. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \mathbf{A}^{\{s,f\}} \cdot  \mathbf{A}^{\{f, f\}} \cdot  \mathbf{A}^{\{f,s\}}  \cdot \mathbf{c}^{\{s\}} = \frac{1}{120} \\
&43. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \mathbf{A}^{\{s,f\}} \cdot  \mathbf{A}^{\{f, s\}} \cdot  \mathbf{A}^{\{s,f\}}  \cdot \mathbf{c}^{\{f\}} = \frac{1}{120} \\
&44. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \mathbf{A}^{\{s,f\}} \cdot  \mathbf{A}^{\{f, s\}} \cdot  \mathbf{A}^{\{s,s\}}  \cdot \mathbf{c}^{\{s\}} = \frac{1}{120} \\
&45. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \mathbf{A}^{\{s,s\}} \cdot  \mathbf{A}^{\{s, f\}} \cdot  \mathbf{A}^{\{f,f\}}  \cdot \mathbf{c}^{\{f\}} = \frac{1}{120} \\
&46. ~~&  \mathbf{b}^{\{s\}}\,^T \cdot \mathbf{A}^{\{s,s\}} \cdot  \mathbf{A}^{\{s, s\}} \cdot  \mathbf{A}^{\{s,f\}}  \cdot \mathbf{c}^{\{f\}} = \frac{1}{120} \\
\end{eqnarray*}

